Gradient Descent for Deep Matrix Factorization: Dynamics and Implicit Bias towards Low Rank

In deep learning, it is common to use more network parameters than training points. In such scenarioof over-parameterization, there are usually multiple networks that achieve zero training error so that thetraining algorithm induces an implicit bias on the computed solution. In practice, (stochastic) gradientdescent tends to prefer solutions which generalize well, which provides a possible explanation of thesuccess of deep learning. In this paper we analyze the dynamics of gradient descent in the simplifiedsetting of linear networks and of an estimation problem. Although we are not in an overparameterizedscenario, our analysis nevertheless provides insights into the phenomenon of implicit bias. In fact, wederive a rigorous analysis of the dynamics of vanilla gradient descent, and characterize the dynamicalconvergence of the spectrum. We are able to accurately locate time intervals where the effective rankof the iterates is close to the effective rank of a low-rank projection of the ground-truth matrix. Inpractice, those intervals can be used as criteria for early stopping if a certain regularity is desired. Wealso provide empirical evidence for implicit bias in more general scenarios, such as matrix sensing andrandom initialization. This suggests that deep learning prefers trajectories whose complexity (measuredin terms of effective rank) is monotonically increasing, which we believe is a fundamental concept for thetheoretical understanding of deep learning.

==> sec_MatrixSensing.tex <==

We will now examine cases where only partial information of the ground truth is given. In general, exact recovery cannot be guaranteed without further assumptions and we do not aim at providing any results comparable to the ones in Section \ref{sec:AnalysisOfDynamics}. %or regularizers, which is not our aim for this section. 
We would rather like to discuss the behavior of gradient descent in such less well-posed settings and draw the reader's attention to certain stumbling blocks one encounters. We consider two types of measurement operators popular in recent literature \cite{li2018algorithmic,gunasekar2017implicit}: Gaussian measurements, which are prototypical for measurements fulfilling a restricted isometry property, in Section \ref{subsec:GaussianMeasurements} and commuting measurements in Section \ref{subsec:CommutingMeasurements}. Recall the definitions of measurement map $\mathcal{A}\colon \mathbb{R}^{n\times n} \rightarrow \mathbb{R}^m$ and loss function $\mathcal{L}\colon \mathbb{R}^{n\times n} \rightarrow \mathbb{R}$ \red{(Ed: maybe we should label one $\mathcal{L}$ as $\mathcal{L}_{\text{simp}}$? J: I'm not sure if it's not just confusing since the loss is not frequently used...)}
%
\begin{align} 
    \square{\mathcal{A}(\W)}_i &= \frac{1}{\sqrt{m}} \inner{A_i}{\W}_F, \label{eq:DefA_Repeated}\\
    \mathcal{L}(\W) &= \frac{1}{2} \norm{\mathcal{A}(\W) - y}{2}^2 \label{eq:L_MatrixSensing_Repeated}.
    % \nabla_\W \mathcal{L}(\W)
    % &= \frac{1}{m}\sum_{i=1}^m \langle A_i, \W - \Wstar \rangle A_i \tag{\ref{eq:Lgrad}}.
\end{align}
We will analyze connections and distinctions between \eqref{eq:DefA_Repeated}-\eqref{eq:L_MatrixSensing_Repeated} and the simplified loss function
\begin{align}
    \mathcal{L}(\W) = \frac{1}{2} \|\W - \Wstar\|_{F}^2 \label{eq:L_MatrixFactorization_Repeated}
\end{align}
that has been considered in the previous sections.

%-------------------------------------------------------------

\subsection{Gaussian Measurement}
\label{subsec:GaussianMeasurements}

%-------------------------------------------------------------

Suppose $A_1,...,A_m$ are $m$ i.i.d. Gaussian matrices. Then the loss function in \eqref{eq:L_MatrixSensing_Repeated} is closely related to the simplified loss function in \eqref{eq:L_MatrixFactorization_Repeated}, in the sense that its expected gradient equals the gradient of \eqref{eq:L_MatrixFactorization_Repeated}. Moreover, the actual gradient of \eqref{eq:L_MatrixSensing_Repeated} concentrates well around its expectation.

\begin{lemma}\label{lem:GaussianConcentration}
    Suppose $A_1,...,A_m$ are independent copies of a Gaussian matrix $A \in\mathbb{R}^{n\times n}$ and consider the loss function $\mathcal{L}$ in \eqref{eq:L_MatrixSensing_Repeated}. Then $\mathbb{E}[\nabla_\W \mathcal{L}(\W)] =\W - \Wstar$.
    %and $\text{Var}[\nabla_\W \mathcal{L}(\W)] = \frac{\|\W - \Wstar\|_F^2}{m}\cdot J$, where $J\in\mathbb{R}^{n\times n}$ is the matrix of ones.
    Moreover, for any $u \ge 0$,
    \begin{equation*}
        \norm{\nabla_\W \mathcal{L}(\W)-(\W-\Wstar)}{F}\le C_1 \sigma^2 \max\{\delta,\delta^2\} \norm{\W-\Wstar}{F}
    \end{equation*}
    with probability at least $1-\exp(-u^2)$, where $\delta = C_2\Big(\sqrt{\frac{n^2}{m}}+\frac{u}{\sqrt{m}}\Big)$, $\sigma^2=\text{Var}(A)$, and $C_1$ and $C_2$ are positive constants.
\end{lemma}
%
\begin{proof}
    Computation of the expectation is straight-forward and thus omitted. Let us identify $\mathbb{R}^{n\times n}$ with $\mathbb{R}^{n^2}$.
    Thus, each $X\in\mathbb{R}^{n\times n} $ is identified with a vectorized version and the measurement map $\mathcal{A}:\mathbb{R}^{n\times n}\rightarrow \mathbb{R}^m$ is identified with a matrix in $\mathbb{R}^{m\times n^2}$. By abuse of notation, we denote this matrix by $\mathcal{A}$ as well and do not distinguish between $X$ and its vectorization. Consequently, $\mathcal{A}^*\big(\mathcal{A}(X)\big)$ is equivalent to $\mathcal{A}
    ^{\top}\mathcal{A} X$. Note that  
    \begin{align*}
        & \norm{\nabla_\W \mathcal{L}(\W)-(\W-\Wstar)}{F}
        % =  \norm{\text{vec}\big(\nabla_\W\mathcal{L}(\W)\big)-\text{vec}(\W-\Wstar)}{2}\\
        % = & \norm{\frac{1}{m}\mathcal{A}^\top\mathcal{A}(\text{vec}(\W-\Wstar))- (
        % \text{vec}(\W-\Wstar)}{2} 
        % \le  \norm{\frac{1}{m}\mathcal{A}^\top\mathcal{A}-I}{}\norm{\text{vec}(\W-\Wstar)}{2}\\
        % = &
        \leq \norm{\frac{1}{m}\mathcal{A}^\top\mathcal{A}-I}{}\norm{\W-\Wstar}{F}\;.
    \end{align*}
    By a suitable concentration inequality \cite[Theorem 4.6.1]{vershynin_2018} we get, for any $u \ge 0$,
    \begin{equation*}
       \norm{\frac{1}{m}\mathcal{A}^\top\mathcal{A}-I}{}\le  C_1 \sigma^2 \max\{\delta,\delta^2\}
    \end{equation*}
    with probability at least $1-\exp(-u^2)$ with $\delta$ and constants as declared.
\end{proof}
%
%\textcolor{blue}{(Omit proof)} The proof of Lemma \ref{lem:GaussianConcentration} can be found in Section \ref{sec:GaussianProofs}. 
% The proof is straight-forward and thus omitted. Lemma \ref{lem:GaussianConcentration} implies that the expected gradient equals the ideal gradient of \eqref{eq:L_MatrixFactorization_Repeated} establishing a connection to Theorem \ref{theorem:IdenticalInitialization_ContinuousNonAsymptoticRate}.
%
However, Lemma \ref{lem:GaussianConcentration} does not imply that throughout iterations the trajectory of gradient descent based on \eqref{eq:L_MatrixSensing_Repeated} remains close to the trajectory based on \eqref{eq:L_MatrixFactorization_Repeated}. The difference, though being small at each step, can grow exponentially in time. Although such growth has not been observed in our experiments, it remains a theoretical challenge to bound the difference of all iterates. Therefore, the community often considers commuting measurements, which are less general but more favorable in terms of algebraic structure, as a natural precursor when approaching theoretical analysis.
%
% Note that direct computation of an expected trajectory of the gradient descent iterates $\W_j(\tdisc)$ is difficult due to the lack of stochastic independence between the factor matrices and the gradient. Instead, we complement Lemma \ref{lem:GaussianConcentration} with a corresponding concentration result to emphasize the just conjectured connection to the setting of Theorem \ref{theorem:IdenticalInitialization_ContinuousNonAsymptoticRate}. 
%
% The proof of Lemma \ref{lem:GaussianConcentration} can be found in Section \ref{sec:GaussianProofs}. Both results together, Lemmas \ref{lem:GaussianConcentration} and \ref{lem:GaussianConcentration}, suggest that, for $m$ sufficiently large, Theorem \ref{theorem:IdenticalInitialization_ContinuousNonAsymptoticRate} still yields an accurate description of gradient descent. 
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commuting Measurements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Commuting Measurement}
\label{subsec:CommutingMeasurements}

Due to its favorable algebraic structure, the setting of commuting measurements, i.e., all measurement matrices $A_1,...,A_m$ commute with each other, is popular in common literature, cf.\ \cite{gunasekar2017implicit}. In what follows, we further restrict ourselves to symmetric measurement matrices, so that $A_1,...,A_m$ are simultaneously diagonalizable by an orthogonal matrix $O \in \mathbb{R}^{n\times n}$ and can be written as
% Let us now turn to the second setting which appeared in recent literature \red{REFERENCE}. We first restrict ourselves to commuting symmetric measurement operators $\mathcal{A}$, defined as in \eqref{eq:DefA}, whose component matrices $A_i$, $i \in [m]$, are simultaneously diagonalizable as
\begin{align} \label{eq:CommMeas}
    A_i = O\,\diag(a^{(i)})\,O^\tT
\end{align}
for some $a^{(i)}\in\mathbb{R}^n$, $1\le i\le m$. We refer to $O$ as the underlying orthogonal matrix and to $a^{(1)},...,a^{(m)}$ as the underlying measurement vectors.

%Once again, there is a natural relation to the simplified setting \eqref{eq:L_MatrixFactorization_Repeated}. In the case where $m = n$ and $O$ diagonalizes $\Wstar$, the loss function equals the simplified loss function \eqref{eq:L_MatrixFactorization_Repeated} if we choose $a^{(i)} = n e_i \in \mathbb{R}^n$ (the scaled $i$-th canonical vector). Note that only $n$ measurements are necessary, since parts of $\Wstar$ are already encoded in the measurements themselves and thus assumed as prior knowledge.

%Let us first emphasize that the commuting measurement set-up has a black spot which to the best of our knowledge is hardly discussed in the literature. If $\mathcal{A}$ is constructed from matrices $A_i$ in \eqref{eq:CommMeas}, ground-truth matrices $\Wstar,\Wstar'$ for which $O^\top \Wstar O$ and $O^\top \Wstar' O$ have the same diagonal cannot be distinguished from the measurements and, consequently, the reconstruction (generalization) error will heavily depend on the initialization. Indeed, for any $\Wstar \in \mathbb{R}^{n\times n}$,
%\begin{align*}
%    \mathcal{A} (\Wstar) 
%    &= ( \langle O\,\diag(a^{(i)})\,O^\tT,\Wstar \rangle_F )_{i=1}^m 
%    = ( \langle \diag(a^{(i)}), O^\top \Wstar O \rangle_F )_{i=1}^m \\
%    &= ( \langle a^{(i)}, \diag( O^\top \Wstar O ) \rangle_F )_{i=1}^m.
%\end{align*}

We will see that a proper choice of $O$ (so that $A_i$ and $\Wstar$ are simultaneously diagonalized) is the key assumption for full recovery, but rather unrealistic in practice. Unfortunately, dropping this assumption leads to non-trivial lower bounds of reconstruction error, cf. Proposition \ref{prop:CommutGeneralizationError}, and questions the meaning of existing theoretical results in this setting. Let us emphasize that those lower bounds are restricted to the symmetric case only for the sake of consistency of notation. The arguments extend to general commuting measurements in a straight-forward way. \red{J: Remove next sentence + Lemma 5.2, since it is not really used for deriving Proposition 5.3?} In the symmetric setting, however, we can explicitly analyze the corresponding dynamics in accordance with the analysis of Section \ref{sec:AnalysisOfDynamics} to highlight parallels as well as differences.
%
\begin{lemma} \label{lemma: ComMeas: IdenticalInitialization_MatrixDynamics}
Let $A_i = O\,\diag(a^{(i)})\,O^\top$, $i \in [m]$, for some orthogonal matrix $O\in\mathbb{R}^{n\times n}$ and some vectors $a^{(1)},...,a^{(m)} \in \mathbb{R}^n$.
Let $\W_j$ follow the gradient descent dynamics in \eqref{eq:MatrixFactorization_GradientDescent} with identical initialization \eqref{eq:MatrixFactorization_IdenticalInitialization}. 
Then the matrix $\D_j(\tdisc):= O^\tT\W_j(\tdisc)O$ is real, diagonal, identical (i.e., there exists $\D\in \mathbb{R}^{n\times n}$ with $\D_j = \D$ for all $j$), and the $s$-th eigenvalue of $\D$ follows the dynamics
\begin{equation}
\label{eq:ComMeas: Eigenavalue Dynamics}
    \D_{ss}(\tdisc+1) = \D_{ss}(\tdisc) - \eta \D_{ss}(\tdisc)^{N-1}\sum\limits_{l=1}^n c_{sl} (\D_{ll}(\tdisc)^N-\tilde\lambda_{l}).
\end{equation}
where $c_{sl} = \frac{1}{m}\sum\limits_{i=1}^m a^{(i)}_s a^{(i)}_l$ and $\tilde\Lambda \in \mathbb{R}^{n\times n}$ is the diagonal matrix with diagonal $\diag\big(O^\top \Wstar O\big)$ and entries $\tilde{\lambda}_i$, for $i \in [m]$.
\end{lemma}
%
\begin{proof}
Due to initialization via identity matrix, a straightforward inductive argument shows that all $W_i(\tdisc)$ are symmetric and diagonalizable by $O$. As in the proof of Lemma \ref{lemma:IdenticalInitialization_MatrixDynamics} this directly implies all factors being equal. Thus, we can write gradient descent as 
\begin{equation*}
    \W_1(\tdisc+1) = \W_1(\tdisc)-\eta \W_1(\tdisc)^{N-1}\frac{1}{m}\sum_{i=1}^m \langle A_i, \W_1(\tdisc)^N - \Wstar \rangle A_i.
\end{equation*}
Diagonalizing (multiplying with $O^\top$ from the left and $O$ from the right) yields
\begin{align*}
    \D(\tdisc+1) 
    &= \D(\tdisc)-\frac{\eta}{m} \D(\tdisc)^{N-1}\sum_{i=1}^m \langle A_i, \W_1(\tdisc)^N - \Wstar \rangle O^\top A_i O\\
    &= \D(\tdisc)-\frac{\eta}{m} \D(\tdisc)^{N-1}\sum_{i=1}^m \langle A_i, \W_1(\tdisc)^N - \Wstar \rangle \diag\big(a^{(i)}\big)\\
    &= \D(\tdisc)-\frac{\eta}{m} \D(\tdisc)^{N-1}\sum_{i=1}^m \text{Tr}\big[\diag\big(a^{(i)}\big) \big(\D^N(\tdisc)-O^\top\Wstar O\big)\big] \diag\big(a^{(i)}\big)\\
    &= \D(\tdisc)-\frac{\eta}{m} \D(\tdisc)^{N-1}\sum_{i=1}^m \sum\limits_{l=1}^n a^{(i)}_l \big(\D_{ll}^N(\tdisc)-\tilde\lambda_l\big) \diag\big(a^{(i)}\big).
\end{align*}
Since $\D(\tdisc+1)$ is also diagonal, the conclusion follows from restricting to the diagonal entries.
% \begin{align*}
%     & O^\top \mathcal{A}^{*}\big(\mathcal{A}(\W_1^N(\tdisc)-\Wstar)\big) O \\
%     = & \sum\limits_{i=1}^m \diag\big(a^{(i)}\big) \text{Tr}\big(A_i^\top \big(\W_1^N-\Wstar\big)\big)\\
%     = & \sum\limits_{i=1}^m \diag\big(a^{(i)}\big) \text{Tr}\big[\diag\big(a^{(i)}\big) \big(\D^N(\tdisc)-O^\top\Wstar O\big)\big]
% \end{align*}
% which concludes the proof when rewriting 
% \begin{equation*}
%     \text{Tr}\big[\diag\big(a^{(i)}\big) \big(\D^N(\tdisc)-O^\top\Wstar O\big)\big] = \sum\limits_{l=1}^n a^{(i)}_l \big(\D_{ll}^N-\tilde\lambda_l\big)
% \end{equation*}
\end{proof}
%
% \begin{remark}
% Lemma \ref{lemma: ComMeas: IdenticalInitialization_MatrixDynamics} generalizes Lemma \ref{lemma:IdenticalInitialization_MatrixDynamics} since $c_{s l}=\delta_{s l}$ and $\tilde{\Lambda} = \Lambda$, for $O=\V$ and $a^{(i)} = e_i \in \mathbb{R}^n$.
% \end{remark}
%
% \begin{proposition} \label{thm:CommutingEigenbasis}
%     Let $A_i = O\,\diag(a^{(i)})\,O^\top$ $i=1,...,m$ for some orthogonal matrix $O$ and some vectors $a^{(i)}\in \mathbb{R}^n$. Let $\W_j$ be the solution to the gradient descent \eqref{eq:MatrixFactorization_GradientDescent} with identical initialization \eqref{eq:MatrixFactorization_IdenticalInitialization}. Then all iterates $\W(\tdisc)$ are diagonalizable by $O$.
% \end{proposition}
%
\begin{figure}
\centering
\begin{subfigure}[b]{1\textwidth}
   \includegraphics[width=1\linewidth]{Figures_ComMeas/Comparison2_Good.png}
   \caption{Choosing correct eigenvectors $O=\V$.}
   \label{subfig: Right Eigenvectors} 
\end{subfigure}
\begin{subfigure}[b]{1\textwidth}
   \includegraphics[width=1\linewidth]{Figures_ComMeas/Comparison2_Bad.png}
   \caption{\textcolor{red}{(Are there better ways to illustrate proposition 5.2?)} Choosing $O$ as in Proposition \ref{prop:CommutGeneralizationError}.}
   \label{subfig: Rotated Eigenvectors}
\end{subfigure}
\caption{Error and Eigenvalue Dynamics using Commuting Measurements}
\small{The figure shows error and eigenvalue dynamics on a ground truth $\Wstar = \diag(5,4,3,2)$ using commuting measurements. In Figure \ref{subfig: Right Eigenvectors} these measurements are given by the outer products $e_1e_1^\top,...,e_n e_n^\top$ where $e_i\in\mathbb{R}^n$ are the canonical vectors. In Figure \ref{subfig: Rotated Eigenvectors} the first two measurements matrices are replaced  $w_1w_1^\top$ and $w_2w_2^\top$ where $w_1,w_2$ are 45 degree rotations of $e_1, e_2$ in the space spanned by these two canonical vectors.
Note that the lower bound for the test error, as computed in Proposition \ref{prop:CommutGeneralizationError}, is illustrated in Figure \ref{subfig: Rotated Eigenvectors}. Further parameters are: $N=3,\,\eta = 10^{-3},\, \alpha = 10^{-2}$. The test error describes the quantity $\norm{\W(\tdisc)-\Wstar}{F}\cdot\norm{\Wstar}{F}^{-1}$ and the training error the quantity $\norm{\mathcal{A}\big(\W(\tdisc)-\Wstar\big)}{2}\cdot\norm{y}{2}^{-1}$.
% Note that in \ref{subfig: Rotated Eigenvectors} the first two eigenvalues are identical and converge to the average of $\lambda_1$ and $\lambda_2$. This is caused by the 45-degree rotation which causes the imposed eigenvectors $w_1, w_2$ to lie exactly in between the original eigenvectors $e_1,e_2$. \
}
\label{fig: Comparing rotated eigenvector an original eigenvectors}
\end{figure}
%
Lemma \ref{lemma: ComMeas: IdenticalInitialization_MatrixDynamics} shows that $\W$ remains diagonalizable by $O$ in all iterations. In other words, when initializing with identity, the best solution one can hope for is 
\begin{equation}\label{eq:CommutingOptimizationIdentical}
    \arg\min_{\W \in \mathbb{R}^{n\times n}} \|\W-\Wstar\|_F^2, \quad \text{ s.t. } \W = O\D O^\top \text{ for some diagonal }\D.
\end{equation}
Such minimizers in general do not, and in fact cannot, coincide with $\W$ because \eqref{eq:ComMeas: Eigenavalue Dynamics} shows that the dynamics depend only on the diagonal of $O^\top \Wstar O$ but not its off-diagonal terms.
Clearly, if the matrix $O^\top \Wstar O$ has relevant off-diagonal terms, there is loss of information rendering exact recovery impossible without further assumptions. The situation hardly improves if we consider small random initializations instead of the identical initialization.
%
%
% \begin{remark}
%   Note that the Lemma \ref{lem: Worst-Case Scenario} could have been stated more rigorously. The above formulation, however, respects the ability of gradient descent to change the order of eigenvalues during optimization (c.f. coupling of eigenvalue dynamics in lemma \ref{lemma: ComMeas: IdenticalInitialization_MatrixDynamics}).
% \end{remark}
%
%---------------Work in Progress-----------------
\begin{proposition} \label{prop:CommutGeneralizationError}
    \textcolor{red}{Please check $\rightarrow$ wrong... Has to be worked over or removed... I think using Corollary 1 in \cite{arora2019implicit} can be used to get the statement for the trajectory of the flow!}
    Let $\Wstar \in \mathbb{R}^{n\times n}$ with eigenvalue decomposition $\Wstar = \V\Dground\V^\top$ be given and assume w.l.o.g.\ that $\Dground_{11}$ is separated from the remaining spectrum of $\Wstar$ by $\delta$, where
    \begin{equation}\label{eq:SpctrumGapMax}
        \delta := \max\limits_{j} \min\limits_{i\neq j} \big|\Dground_{ii}-\Dground_{jj}\big| > 0.
    \end{equation}
    Let $\W_j$ follow the gradient descent dynamics in \eqref{eq:MatrixFactorization_GradientDescent} with $\mathcal{L}$ as in \eqref{eq:L_MatrixSensing_Repeated} and commuting measurements $\mathcal{A}$ with underlying orthogonal matrix $O= \big(o_1\big|...\big|o_n\big)$. Denote the minimal angle between the $j$-th eigenvector of $V$ and $O$ by
    \begin{equation}\label{eq:EigenspaceAngle}
        \gamma_j := \min\limits_{i=1,...,n} \angle\big(v_{j}, o_i\big)\, \in [0,\frac{\pi}{2}].
    \end{equation}
    where $\angle(x,z) := \arccos{\frac{|\inner{x}{z}|}{\norm{x}{2}\norm{z}{2}}}$, for $x,z\in\mathbb{R}^n$. Then, for any initialization $\W_j(0)$ fulfilling $\|\W\|\leq\alpha$, the approximation error is lower bounded by
    \begin{align*}
        \|\W(\tdisc) - \Wstar\| \ge \frac{\delta}{2}\sin(\gamma_1) - \alpha,
    \end{align*}
    for all $\tdisc$. In particular, for $O = R\V$, where
    \begin{align*}
        R :=  I+\left(\cos\left(\frac{\pi}{4}\right)-1\right)\left(v_1v_1^\top + v_2v_2^\top\right)-\sin\left(\frac{\pi}{4}\right)\left(v_1v_2^\top - v_2v_1^\top\right),
    \end{align*}
    we have, for all $k$,
    \begin{align*}
        \norm{\W(\tdisc) -  \Wstar}{F} \ge \norm{\W(\tdisc) - \Wstar}{} \ge \frac{\delta}{\sqrt{2}} - \alpha.
    \end{align*}
\end{proposition}
%
The proof relies on the following version of the Davis-Kahan $\sin(2\Theta)$-Theorem \cite{davis1970rotation}.
%
\begin{lemma}[{Davis-Kahan $\sin(2\Theta)$-Theorem, \cite[Theorem 4.5.5]{vershynin_2018}}]\label{lem: Worst-Case Scenario}
    Let $\Wstar = \V\Dground \V^\top \in \mathbb{R}^{n\times n}$. Assume that there is at least one eigenvalue well separated from the remaining spectrum by $\delta$ in \eqref{eq:SpctrumGapMax}. Let further $j^*$ be the corresponding maximizing index and $v_{j^*}$ the corresponding eigenvector.     
    Then, for any matrix $Z$ with eigenvectors $o_1,...,o_n$ we have:
    %
    \begin{equation*}
        \norm{Z-\Wstar}{}\ge \frac{\delta}{2}\sin(\gamma_{j^*})\;,
    \end{equation*}
    where $\gamma_{j}$ is defined in \eqref{eq:EigenspaceAngle}.
\end{lemma}
%
\begin{proof}[Proof of Proposition \ref{prop:CommutGeneralizationError}]
    Since all measurements are diagonalizable by $O$, the gradient $\nabla\W_j(\tdisc)$ in \eqref{eq:Lgrad}
    \begin{align*}
        \nabla_{\W_j} \mathcal{L}(\W(k))
        = \mathcal{A}^*( \mathcal{A}(\W) - y )
        = \frac{1}{m}\sum_{i=1}^m (\langle A_i, \W \rangle - y_i)A_i
        = \frac{1}{m}\sum_{i=1}^m \langle A_i, \W - \Wstar \rangle A_i.
    \end{align*} 
    is diagonalized by $O$, for all $\tdisc$. Hence $\W(\tdisc)$ can be written as $\W(0)+O\D(\tdisc) O^\top$ and Lemma \ref{lem: Worst-Case Scenario} yields
    \begin{align*}
        \|\W(\tdisc) - \Wstar\|
        &= \|\W(0)+O\D(\tdisc) O^\top - \V\Dground\V^\top\|\\
        &\geq \|O\D(\tdisc) O^\top - \V\Dground\V^\top\| - \|\W(0)\|
        \geq \frac{\delta}{2}\sin(\gamma) - \alpha.
    \end{align*}
    The second claim follows since the inner product between columns of $O = RV$ and $v_1$ is
    \begin{equation*}
        \big|\inner{o_i}{v_1}\big| = \big|\inner{v_i}{R^\top v_1}\big| =
            \begin{cases}
                 0\, &\textrm{ if } i>2\\
                 \sin(\frac{\pi}{4})\, &\textrm{ if } i=2\\
                 \cos(\frac{\pi}{4})\, &\textrm{ if } i=1\\
            \end{cases}
    \end{equation*}
    Thus, the minimal angle between $v_1$ and the columns of $O$ is $\frac{\pi}{4}$.
\end{proof}
%
%, because the problem simply becomes
%\begin{equation}\label{eq:CommutingOptimizationRandom}
%    \arg\min_{\W \in \mathbb{R}^{n\times n}} \|\W(0)+\W-\Wstar\|_F^2 \quad \text{ s.t. } \W = O\D O^\top \text{ for some diagonal }\D.
%\end{equation}
%When the initialization lies close to zero, a common scaling in the literature \textcolor{red}{REFERENCE}, %\eqref{eq:CommutingOptimizationRandom} is essentially equivalent to \eqref{eq:CommutingOptimizationIdentical} and lower bounds on the reconstruction error are comparable.
Proposition \ref{prop:CommutGeneralizationError} shows that, for the in literature common scaling $\alpha \ll 1$ \cite{gunasekar2017implicit,li2018algorithmic,Bach2019implicit}, the generalization error is of the order of the maximal spectral gap of $\Wstar$ if $\mathcal{A}$ is not constructed under knowledge of its eigenspaces.
%The following specific poor choice of $\mathcal{A}$ gives a lower bound of the worst-case scenario.
%
% with entries $\tilde{\lambda}_i$, for $i \in [m]$. While $\Lambda \neq \tilde{\Lambda}$ in general,
% \begin{equation*}
%     \min_{i \in [m]} \lambda_i \le \min_{i \in [m]} \tilde\lambda_i \le \max_{i \in [m]} \tilde\lambda_i \le \max_{i \in [m]} \lambda_i \;,
% \end{equation*}
% by the Courant-Fisher theorem and
% \begin{equation*}
%     \sum\limits_{i=1}^n\lambda_i = \sum\limits_{i=1}^n\tilde\lambda_i
% \end{equation*}
% which, for positive semi-definite $\Wstar$, means that nuclear norm is preserved. This relation, see Figure \ref{fig: Comparing rotated eigenvector an original eigenvectors} for illustration, is not surprising. Since $\W$ minimizes $\|\W-\Wstar\|$ subject to $\W = O \diag(\lambda_i) O^\top$, its performance generalization error highly depends on the choice of $O$ and might be significant if the spectrum admits at least two separated clusters of eigenvalues. Though bound to the eigenbasis $O$, gradient descent approximates $\Wstar$ best possible. Unfortunately, as the following negative result shows, this still causes an unsatisfactory generalization error if the spectrum admits at least two separated clusters of eigenvalues and $O$ is chosen in a malicious way.%
%
% The proof of proposition \ref{prop:LBgeneralizationError} relies on the following variant of the well known Davis-Kahan $\sin(2\Theta)$-Theorem \cite{davis1970rotation}.
%
%---------------Work in Progress-----------------
%
%\begin{proposition} \label{prop:LBgeneralizationError}
%    Let $\Wstar \in \mathbb{R}^{n\times n}$ with eigenvalue decomposition $\Wstar = \V\Dground\V^\top$ be given and assume w.l.o.g.\ that $\Dground_{11}$ is separated from the remaining spectrum of $\Wstar$ by $\delta$ as in \eqref{eq:SpctrumGapMax}.    Define 
%    \begin{align*}
%        R := & I+\left(\cos\left(\frac{\pi}{4}\right)-1\right)\left(v_1v_1^\top + v_2v_2^\top\right)-\sin\left(\frac{\pi}{4}\right)\left(v_1v_2^\top - v_2v_1^\top\right)\;
%    \end{align*}
%    to be a rotation matrix in the two dimensional subspace of $\mathbb{R}^n$ that is spanned by the two eigenvectors $v_1,v_2$. Then, for a commuting measurement operator $\mathcal{A}$ with underlying orthogonal matrix $O = R\V$ and any initialization $\W_j(0)$ fulfilling $\|\W\|\leq\alpha$, gradient descent fulfills
%    \begin{align*}
%        \norm{\W(\tdisc) -  \Wstar}{F} \ge \norm{\W(\tdisc) - \Wstar}{} \ge \frac{\delta}{\sqrt{2}} - \alpha.
%    \end{align*}
%\end{proposition}
%
%\begin{proof}
%    Just observe that the inner product between the columns of the orthogonal matrix $O$ and $v_1$ are
%    \begin{equation*}
%        \big|\inner{o_i}{v_1}\big| = \big|\inner{v_i}{R^\top v_1}\big| =
%            \begin{cases}
%                 0\, &\textrm{ if } i>2\\
%                 \sin(\frac{\pi}{4})\, &\textrm{ if } i=2\\
%                 \cos(\frac{\pi}{4})\, &\textrm{ if } i=1\\
%            \end{cases}
%    \end{equation*}
%    Thus, the minimal angle between $v_1$ and the columns of $O$ is $\frac{\pi}{4}$. Proposition \ref{prop:CommutGeneralizationError} now yields the claim.
%\end{proof}
%
An interesting question is, how the lower bound in Proposition \ref{prop:CommutGeneralizationError} behaves if $O$ is chosen at random. Explicit lower bounds of the generalization error depend on spectral gaps of $\Wstar$ and angles between the eigenspace of $\Wstar$ and the eigenspace of $A_1,...,A_m$ such that further considerations in this direction involve in-depth application of Haar-distribution theory and would go beyond the scope of this work. Nevertheless, it is easy to see that for randomly chosen $O$ the generalization error is almost surely positive under similar assumptions as in Proposition \ref{prop:CommutGeneralizationError}.
%
\begin{lemma}\label{lemma: ComMeas: Random O full rank}
    Let $O$ be drawn uniformly at random (with respect to the Haar measure) from the set $\mathbb{O}(n) \subset \mathbb{R}^{n\times n}$ of orthogonal matrices and let $A_i = O\,\text{diag}\big(a^{(i)}\big)\,O^\top$, for some $a^{(i)}\in \mathbb{R}^n$ and $i\in [m]$. Then, as long as $\Wstar \neq 0$, the gradient descent limit $\W(\infty) = \lim_{\tdisc \rightarrow \infty} \W(\tdisc)$ %\red{Then, as long as $\Wstar \neq 0$, $\tilde\Lambda$ as defined in section \ref{sec:CommutingMeasurements}} 
    almost surely has full rank. Furthermore, if $\Wstar$ has at least one well separated eigenvalue, the generalization error is almost surely positive.
\end{lemma}
%
\begin{proof}
To see the first property, note that
\begin{align*}
     O^\top \Wstar O
    = O^\top \V \Dground \V^\top O 
    =  Z \Dground Z^\top
    =  \sum\limits_{j=1}^n \Dground_{jj}z_j z_j^\top, 
\end{align*}
where $Z:= O^\top \V\sim O^\top$ by invariance of the Haar-measure.
Hence,
\begin{equation*}
    \tilde\lambda_i = \Big(O^\top \Wstar O\Big)_{ii}= \sum\limits_{j=1}^n \Dground_{jj} z_{ij}^2
\end{equation*}
It is clear that as long as one $\Dground_{jj} \neq 0$ the set of matrices yielding entries $\tilde\lambda_i = 0$ has measure zero. The second property follows again from the Davis-Kahan $\sin(2\Theta)$-Theorem \cite{davis1970rotation}.
\end{proof}
%
%Explicit lower bounds of the generalization error depend on spectral gaps of $\Wstar$ and angles between the eigenspace of $\Wstar$ and the eigenspace of $A_1,...,A_m$.%, which can be complicated without providing considerably deeper insight than the above results.
% proves difficult. Calculating the expected angles between the columns of $O$ and $V$ needs the inner products $\inner{o_i}{v_j}$, for all $i,j$, i.e., one asks for the maximum entry of a Haar distributed matrix.
%and will not be applied here.
%Respective existing results are mainly asymptotic \cite{jiang2005maxima}) 
%Further considerations in this direction involve in-depth application of Haar-distribution theory and would go beyond the scope of this work.
% Appendix \ref{sec:MatrixSensingExample} contains some further discussion on the topic. \red{Remove last sentence + Appendix?}

==> sec_Setting.tex <==

In the following, we will consider two widely known problems in which gradient descent exhibits implicit bias: matrix factorization and matrix sensing \cite{arora2019implicit,Bach2019implicit,gunasekar2017implicit,li2018algorithmic}. In both cases one is interested in finding low-rank solutions, be it to remove noise, to reduce complexity, or to allow unique reconstruction from sub-sampled measurements.

\paragraph{Matrix factorization.} The main challenge of matrix factorization lies in approximating a given matrix $\Wstar \in \mathbb{R}^{n\times n}$ (here and in the following we will restrict ourselves to square matrices) by a matrix product of less complexity, e.g., lower rank, which is cheaper to store and easier to interpret. If the matrix is of the form $\Wstar = \W_\text{LC} + \Xi$, where $\W_\text{LC}$ is a ground-truth of low complexity and $\Xi \in \mathbb{R}^{n\times n}$ is additive noise \textcolor{red}{(need to be more specific in terms of SNR, rather just saying one is signal and one is noise.)}, matrix factorization in addition allows denoising of $\W_\text{LC}$. When considering rank as a measure of complexity, Principal Component Analysis (PCA) may be seen as a prime example \cite{wold1987principal}. PCA approximates $\Wstar$ by a product $\widehat{U} \widehat{V}^\tT$ of two lower-dimensional matrices $\widehat{U},\widehat{V} \in \mathbb{R}^{n\times r}$ such that $\widehat{U} \widehat{V}^\tT$ is or rank at most $r$ and minimizes the Frobenius error $(U,V) \mapsto \|UV^\tT - \Wstar\|_F^2$ (best rank-$r$ term approximation of $\Wstar$). Interestingly, recent research \cite{Bach2019implicit} suggests that a similar solution can be computed by writing $\W = \W_1 \W_2$, for $\W_1, \W_2 \in \mathbb{R}^{n\times n}$, and applying vanilla gradient descent to
\begin{align} \label{eq:L_MatrixFactorization}
    \mathcal{L}(\W) = \frac{1}{2} \norm{\W - \Wstar}{F}^2,
\end{align}
i.e., performing the iterations
\begin{align} 
    \W_{j}(\tdisc+1)
    &= \W_{j}(\tdisc) - \eta \nabla_{\W_{j}}%(\tdisc)} 
    \mathcal{L}(\W(\tdisc))
    \label{eq:MatrixFactorization_GradientDescent}\\
    \W_{j}(0)
    &= \alpha I, \label{eq:MatrixFactorization_IdenticalInitialization}
\end{align}
for $\alpha,\eta > 0$ chosen sufficiently small and an appropriate maximum number of iterations $T$. This is remarkable since neither $\mathcal{L}$ nor the dimensional setting of $\W_1, \W_2$ enforce any low-rankness on $\W(\tdisc) = \W_1(\tdisc)\W_2(\tdisc)$. In connection to recent advances on (linear) neural networks \cite{arora2019implicit} it was even observed that higher order factorizations $\W = \W_1 \cdots \W_N$ can strengthen the regularizing effect. Note that the gradient of $\mathcal{L}$ with respect to a single factor $\W_j$ is given by
\begin{align} \label{eq:L_gradient}
    \nabla_{\W_j} \mathcal{L}(\W) = (\W_1\cdots \W_{j-1})^{\tT} \nabla_{\W} \mathcal{L}(\W) (\W_{j+1}\cdots \W_{N})^{\tT}.
\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Matrix Sensing Setting 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Matrix sensing.} \textcolor{red}{(Move this part (including related Figures) in compact form to Outlook or Numerics?)} In contrast to matrix factorization, matrix sensing is about reconstructing the ground-truth $\Wstar$ from sub-sampled measurements $y = \mathcal{A}(\Wstar) \in \mathbb{R}^m$, $m < n^2$, where the linear operator $\mathcal{A} \colon \mathbb{R}^{n\times n} \rightarrow \mathbb{R}^m$ can be characterized by $m$ matrices $A_i \in \mathbb{R}^{n\times n}$ via
\begin{align} \label{eq:DefA}
    \square{\mathcal{A}(\W)}_i = \frac{1}{\sqrt{m}} \inner{A_i}{\W}_F
\end{align}
and the scaling factor $\frac{1}{\sqrt{m}}$ might be replaced by an arbitrary constant. Based on compressed sensing, cf.\ \cite{foucart:2013} and references therein, a rich theory on matrix sensing has been developed in the last decade, showing unique identification and recovery of rank-$r$ matrices $\Wstar$ from $y$ if $\mathcal{A}$ is suitably chosen and $m \ge C rn$, for some absolute constant $C > 0$. Consequently, if $r \ll n$, reliable reconstruction of $\Wstar$ is possible for $m \ll n^2$.
%satisfies the following property.
%
%\begin{definition}\textcolor{red}{(We probably don't need to define it so precisely since we never really use this definition.)}
%    A linear operator $\mathcal{A} \colon \mathbb{R}^{n\times n} \rightarrow \mathbb{R}^m$ satisfies the \emph{$(r,\delta)-$restricted isometry property (RIP)} if there exists $\delta \in (0,1)$ such that
%    \begin{align*}
 %       (1-\delta) \norm{Z}{F} \le \norm{\mathcal{A}(Z)}{2} \le (1+\delta) \norm{Z}{F},
 %   \end{align*}
 %   for all $Z \in \mathbb{R}^{n\times n}$ of rank at most $r$.
%\end{definition}
%
In particular, operators $\mathcal{A}$ fulfilling \emph{restricted isometry properties (RIPs)} \cite{foucart:2013} allow to reach optimal sample complexities.\\
%which means that if $r \ll n$, reliable reconstruction of $\Wstar$ is possible for $m \ll n^2$.\\ 
While the original works mainly examined regularization procedures to find minimal rank solutions fulfilling the measurements, recent research (motivated by the success of deep neural networks) is focusing on the implicit regularization of gradient descent \cite{gunasekar2017implicit,li2018algorithmic}. To be precise, one is interested in recovering $\Wstar$ from $y$
by minimizing
\begin{align} \label{eq:L_MatrixSensing}
    \mathcal{L}(\W) = \frac{1}{2} \norm{\mathcal{A}(\W) - y}{2}^2
\end{align}
via gradient descent. By abuse of notation we will not distinguish between \eqref{eq:L_MatrixFactorization} and \eqref{eq:L_MatrixSensing}; it is always clear from the context which functional we refer to. As above the trick lies in factorizing $\W$ as $\W_1 \cdots \W_N$ and applying gradient descent to the single factors to implicitly enforce low-rankness. By using that
\begin{align} \label{eq:Lgrad}
    \nabla_\W \mathcal{L}(\W)
    = \mathcal{A}^*( \mathcal{A}(\W) - y )
    = \frac{1}{m}\sum_{i=1}^m (\langle A_i, \W \rangle - y_i)A_i
    = \frac{1}{m}\sum_{i=1}^m \langle A_i, \W - \Wstar \rangle A_i.
\end{align}
\textcolor{red}{(Do we really need to mention RIP here? We never use this later on and it is quite irrelevant to our work.)} It is straight-forward to adapt \eqref{eq:MatrixFactorization_GradientDescent}-\eqref{eq:L_gradient} to the matrix sensing setting. Note that if $\mathcal{A}$ satisfies the $(r,\delta)$-low rank RIP, i.e., 
\begin{align*}
       (1-\delta) \norm{Z}{F} \le \norm{\mathcal{A}(Z)}{2} \le (1+\delta) \norm{Z}{F},
\end{align*}
for all $Z \in \mathbb{R}^{n\times n}$ of rank at most $r$, then
\begin{align} \label{eq:GradientRelation}
    \left\|\nabla_\W \mathcal{L}(\W) - (\W - \Wstar)\right\| \leq \delta \|\W - \Wstar\|_F
\end{align}
for all $\W,\Wstar$ of rank at most $r$. Since RIPs of $\mathcal{A}$ play a central role in recent results on gradient descent for matrix sensing, equation \eqref{eq:GradientRelation}, which under RIP connects the gradient for matrix sensing with the gradient in matrix factorization, motivates us to mainly focus here on the more accessible setting of matrix factorization, see Sections \ref{sec:EffectiveRank} and \ref{sec:AnalysisOfDynamics}, while restricting our treatment of matrix sensing to providing several useful and illustrative insights, see Section \ref{sec:MatrixSensing}. Let us emphasize that we restrict ourselves to symmetric ground-truths $\Wstar \in \mathbb{R}^{n\times n}$ here and in the following. This allows us to derive an accurate description of gradient descent providing valuable insight in the implicit regularization phenomenon. Transferring the results to more general settings is a natural next step (though difficult to perform without giving up on preciseness).

In Figure \ref{fig:Gaussian_m} we can see that as the number of measurements $m$ increases, the trajectory of \eqref{eq:L_MatrixSensing} is getting closer to that of \eqref{eq:L_MatrixFactorization}. This supports the claimed equivalence between \eqref{eq:L_MatrixSensing} and \eqref{eq:L_MatrixFactorization}, for sufficiently large $m$.
%
\begin{figure}
\begin{subfigure}[c]{0.45\textwidth}
\includegraphics[width=\textwidth]{FiguresPython/Gaussian/MoreRuns_highlighted/effRank_gaussian.png}
\subcaption{Effective rank $\norm{\W(\tdisc)}{*}/\norm{\W(\tdisc)}{}$}
\label{subfig:Gaussian_m20}
\end{subfigure} \quad
\begin{subfigure}[c]{0.45\textwidth}
\includegraphics[width=\textwidth]{FiguresPython/Gaussian/MoreRuns_highlighted/Testerror_gaussian.png}
\subcaption{Approximation error $\|\W(\tdisc)-\Wstar\|_F\|\Wstar\|_{F}^{-1}$}
\label{subfig:Gaussian_m100}
\end{subfigure}
\caption{Above are experiments of matrix sensing with $m$ Gaussian measurements. The curve denoted by $m = \infty$ corresponds to gradient descent run on the expected gradient, which according to lemma \ref{lem:GaussianConcentration} equals to the gradient of \eqref{eq:L_MatrixFactorization}. Despite the randomness in measurements, the waterfall phenomenon (multiple plateaus) can be observed and is more obvious as $m$ increases. 
% Setting: $\Wstar\in \mathbb{R}^{10 \times 10}$ with rank $5$ and positive eigenvalues $20,10,5,2,1$. $N=3, \alpha  = 0.1, \eta = 10^{-4}$. The underlying standard deviation of the gaussian measurement matrices is $ \sigma = 0.1$.
}
\label{fig:Gaussian_m}
\end{figure}
%

%
\begin{figure}
\begin{subfigure}[c]{0.45\textwidth}
\includegraphics[width=\textwidth]{FiguresPython/Gaussian/MoreRuns_highlighted/Gaussian_n20_N2_s10.png}
\subcaption{$N=2$}
\label{subfig:Gaussian_N2_sufficient measurements}
\end{subfigure}
\begin{subfigure}[c]{0.45\textwidth}
\includegraphics[width=\textwidth]{FiguresPython/Gaussian/MoreRuns_highlighted/Gaussian_n20_N3_s10.png}
\subcaption{$N=3$}
\label{subfig:Gaussian_N3_sufficient measurements}
\end{subfigure}
\caption{Here the ground truth $\Wstar\in\mathbb{R}^{20\times 20}$ is of rank $r = 2,3,4$. We can see that as $m$ increases, the approximation error decreases. Moreover, as $N$ in creases, such transition becomes more obvious. The drops for $N=3$ happen around $m = 90,120,170$, consistent with the scaling $cnr$.}
\end{figure}
%
\begin{figure}
\begin{subfigure}[c]{0.45\textwidth}
\includegraphics[width=\textwidth]{FiguresPython/Gaussian/MoreRuns_highlighted/Gaussian_n20_N234_r2.png}
\subcaption{Approximation error}
\label{subfig:Gaussian_N234_approx_error}
\end{subfigure}
\begin{subfigure}[c]{0.45\textwidth}
\includegraphics[width=\textwidth]{FiguresPython/Gaussian/MoreRuns_highlighted/Gaussian_n20_N234_r2_prob.png}
\subcaption{Recovery probability (Error less than $0.01$)}
\label{subfig:Gaussian_N234_recover_probability}
\end{subfigure}
\caption{Here the ground truth $\Wstar\in\mathbb{R}^{20\times 20}$ is of rank $2$. The simulations suggest that deeper factorization exhibits a faster and sharper transition. However, it might perform worse in certain regime, depending on the number of samples.}
\label{fig:Gaussian_N234_sufficient_measurements}
\end{figure}
%
\begin{figure}
\includegraphics[width=0.5\textwidth]{FiguresPython/Completion_n20_N234_r2_prob_IRLS.png}
\caption{For matrix completion, the threshold is larger for $N=3,4$ but smaller for $N=2$. It has similar but slightly worse performance compared to IRLS.}
\label{fig:Completion_N234_sufficient_measurements}
\end{figure}
%
